Notes on Pointwise Finite-Dimensional $2$-Parameter Persistence Modules

In this paper, we study pointwise finite-dimensional (p.f.d.) $2$-parameter persistence modules where each module admits a finite convex isotopy subdivision. We show that a p.f.d. $2$-parameter persistence module $M$ (with a finite convex isotopy subdivision) is isomorphic to a $2$-parameter persistence module $N$ where the restriction of $N$ to each chamber of the parameter space $(\mathbb{R},\leq)^2$ is a constant functor. Moreover, we show that the convex isotopy subdivision of $M$ induces a finite encoding of $M$. Finally, we prove that every indecomposable thin $2$-parameter persistence module is isomorphic to a polytope module.

==> app.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for WENWEN LI at 2023-03-09 22:18:10 -0600 


%% Saved with string encoding Unicode (UTF-8) 



@article{dover2013homeomorphism,
	Author = {Dover, James and {\"O}zaydin, Murad},
	Journal = {IMRN: International Mathematics Research Notices},
	Number = {20},
	Title = {Homeomorphism types of restricted configuration spaces of metric graphs.},
	Volume = {2018},
	Year = {2018}}

@article{li2023persistent,
  title={Persistent Homology of Configuration Spaces of Trees},
  author={Li, Wenwen},
  eprint={2310.05303},
  archivePrefix={arXiv},
  year={2023}
}


@article{abrams2002finding,
	Author = {Abrams, Aaron and Ghrist, Robert},
	Journal = {The American mathematical monthly},
	Number = {2},
	Pages = {140--150},
	Publisher = {Taylor \& Francis},
	Title = {Finding topology in a factory: configuration spaces},
	Volume = {109},
	Year = {2002}}

@article{ghrist2008barcodes,
  title={Barcodes: the persistent topology of data},
  author={Ghrist, Robert},
  journal={Bulletin of the American Mathematical Society},
  volume={45},
  number={1},
  pages={61--75},
  year={2008}
}

@article{BL15,
	Author = {Bauer, Ulrich and Lesnick, Michael},
	Journal = {arXiv preprint arXiv:1311.3681},
	Title = {Induced matchings and the algebraic stability of persistence barcodes},
	Year = {2013}}

@article{Botman-2015,
	Author = {Botnan, Magnus},
	Journal = {Proceedings of the American Mathematical Society},
	Number = {8},
	Pages = {3571--3577},
	Title = {Interval decomposition of infinite zigzag persistence modules},
	Volume = {145},
	Year = {2017}}



@article{B2014,
	Author = {Bubenik, Peter and Scott, Jonathan A},
	Journal = {Discrete \& Computational Geometry},
	Number = {3},
	Pages = {600--627},
	Publisher = {Springer},
	Title = {Categorification of persistent homology},
	Volume = {51},
	Year = {2014}}

@article{BE-2020,
	Author = {Buchet, Micka{\"e}l and Escolar, Emerson G},
	archivePrefix={arXiv},
    eprint={2008.00063},
	Title = {The whole in the parts: Putting $n$D persistence modules inside indecomposable $(n+1)$D ones},
	Year = {2020}}

@article{BE-2019,
	Author = {Buchet, Micka{\"e}l and Escolar, Emerson G},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {387--424},
	Publisher = {Springer},
	Title = {Every $1$D persistence module is a restriction of some indecomposable $2$D persistence module},
	Volume = {4},
	Year = {2020}}

@article{CZ2009,
	Author = {Carlsson, Gunnar and Zomorodian, Afra},
	Journal = {Discrete \& Computational Geometry},
	Number = {1},
	Pages = {71--93},
	Publisher = {Springer},
	Title = {The theory of multidimensional persistence},
	Volume = {42},
	Year = {2009}}

@article{zomorodian2005computing,
	Author = {Zomorodian, Afra and Carlsson, Gunnar},
	Journal = {Discrete \& Computational Geometry},
	Number = {2},
	Pages = {249--274},
	Publisher = {Springer},
	Title = {Computing persistent homology},
	Volume = {33},
	Year = {2005}}

@article{2021,
	Author = {Carlsson, Gunnar and Dwaraknath, Anjan and Nelson, Bradley J},
	Journal = {arXiv preprint arXiv:1911.10693},
	Title = {Persistent and zigzag homology: A matrix factorization viewpoint},
	Year = {2019}}

@article{CV-2008,
	Author = {Carlsson, Gunnar and De Silva, Vin},
	Journal = {Foundations of computational mathematics},
	Number = {4},
	Pages = {367--405},
	Publisher = {Springer},
	Title = {Zigzag persistence},
	Volume = {10},
	Year = {2010}}

@inproceedings{CVD,
	Author = {Carlsson, Gunnar and De Silva, Vin and Morozov, Dmitriy},
	Booktitle = {Proceedings of the twenty-fifth annual symposium on Computational geometry},
	Pages = {247--256},
	Title = {Zigzag persistent homology and real-valued functions},
	Year = {2009}}

@article{CV-2011,
	Author = {Tausz, Andrew and Carlsson, Gunnar},
	Journal = {arXiv preprint arXiv:1108.3545},
	Title = {Applications of zigzag persistence to topological data analysis},
	Year = {2011}}

@article{crawley2015decomposition,
	Author = {Crawley-Boevey, William},
	Journal = {Journal of Algebra and its Applications},
	Number = {05},
	Pages = {1550066},
	Publisher = {World Scientific},
	Title = {Decomposition of pointwise finite-dimensional persistence modules},
	Volume = {14},
	Year = {2015}}

@article{botnan2020decomposition,
  title={Decomposition of persistence modules},
  author={Botnan, Magnus and Crawley-Boevey, William},
  journal={Proceedings of the American Mathematical Society},
  volume={148},
  number={11},
  pages={4581--4596},
  year={2020}
}



@article{CSEH2007,
	Author = {Cohen-Steiner, David and Edelsbrunner, Herbert and Harer, John},
	Journal = {Discrete \& computational geometry},
	Number = {1},
	Pages = {103--120},
	Publisher = {Springer},
	Title = {Stability of persistence diagrams},
	Volume = {37},
	Year = {2007}}

@phdthesis{Dee,
	Author = {Deeley, Kenneth},
	School = {Durham University},
	Title = {Configuration spaces of thick particles on graphs},
	Year = {2011}}

@article{MM17,
	Author = {Meehan, Killian and Meyer, David},
	Journal = {arXiv preprint arXiv:1710.02858},
	Title = {An isometry theorem for generalized persistence modules},
	Year = {2017}}

@article{L15,
	Author = {Lesnick, Michael},
	Journal = {Foundations of Computational Mathematics},
	Number = {3},
	Pages = {613--650},
	Publisher = {Springer},
	Title = {The theory of the interleaving distance on multidimensional persistence modules},
	Volume = {15},
	Year = {2015}}

@article{MK2018,
	Author = {Kim, Woojin and M{\'e}moli, Facundo},
	Journal = {Journal of Applied and Computational Topology},
	Number = {4},
	Pages = {533--581},
	Publisher = {Springer},
	Title = {Generalized persistence diagrams for persistence modules over posets},
	Volume = {5},
	Year = {2021}}

@article{otter2017roadmap,
	Author = {Otter, Nina and Porter, Mason A and Tillmann, Ulrike and Grindrod, Peter and Harrington, Heather A},
	Journal = {EPJ Data Science},
	Pages = {1--38},
	Publisher = {Springer},
	Title = {A roadmap for the computation of persistent homology},
	Volume = {6},
	Year = {2017}}

@article{chazal2017introduction,
	Author = {Chazal, Fr{\'e}d{\'e}ric and Michel, Bertrand},
	Journal = {arXiv preprint arXiv:1710.04019},
	Title = {An introduction to topological data analysis: fundamental and practical aspects for data scientists},
	Year = {2017}}

@book{2007,
	Author = {Hazewinkel, Michiel and Gubareni, Nadiya and Kirichenko, Vladimir V},
	Publisher = {Springer Science \& Business Media},
	Title = {Algebras, rings and modules},
	Volume = {1},
	Year = {2004}}

@book{erdmann2018algebras,
	Author = {Erdmann, Karin and Holm, Thorsten},
	Publisher = {Springer},
	Title = {Algebras and representation theory},
	Year = {2018}}

@article{carlsson2009topology,
	Author = {Carlsson, Gunnar},
	Journal = {Bulletin of the American Mathematical Society},
	Number = {2},
	Pages = {255--308},
	Title = {Topology and data},
	Volume = {46},
	Year = {2009}}

@inproceedings{carlsson2004persistence,
	Author = {Carlsson, Gunnar and Zomorodian, Afra and Collins, Anne and Guibas, Leonidas},
	Booktitle = {Proceedings of the 2004 Eurographics/ACM SIGGRAPH symposium on Geometry processing},
	Pages = {124--135},
	Title = {Persistence barcodes for shapes},
	Year = {2004}}

@article{krishnan2020invertibility,
	Author = {Krishnan, Sanjeevi and Ogle, Crichton},
	Journal = {arXiv preprint arXiv:2010.11276},
	Title = {Invertibility in Category Representations},
	Year = {2020}}

@article{kocc2020representations,
	Author = {Ko{\c{c}}, Ayten and {\"O}zayd{\i}n, Murad},
	Journal = {Journal of pure and applied algebra},
	Number = {3},
	Pages = {1297--1319},
	Publisher = {Elsevier},
	Title = {Representations of Leavitt path algebras},
	Volume = {224},
	Year = {2020}}

@book{steinberg2016representation,
	Author = {Steinberg, Benjamin},
	Publisher = {Springer},
	Title = {Representation theory of finite monoids},
	Year = {2016}}

@article{patel2018generalized,
	Author = {Patel, Amit},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {397--419},
	Publisher = {Springer},
	Title = {Generalized persistence diagrams},
	Volume = {1},
	Year = {2018}}

@article{alpert2021configuration,
	Author = {Alpert, Hannah and Manin, Fedor},
	Journal = {arXiv preprint arXiv:2107.04574},
	Title = {Configuration spaces of disks in a strip, twisted algebras, persistence, and other stories},
	Year = {2021}}

@article{carlsson2012computational,
	Author = {Carlsson, Gunnar and Gorham, Jackson and Kahle, Matthew and Mason, Jeremy},
	Journal = {Physical Review E},
	Number = {1},
	Pages = {011303},
	Publisher = {APS},
	Title = {Computational topology for configuration spaces of hard disks},
	Volume = {85},
	Year = {2012}}

@article{baryshnikov2014min,
	Author = {Baryshnikov, Yuliy and Bubenik, Peter and Kahle, Matthew},
	Journal = {International Mathematics Research Notices},
	Number = {9},
	Pages = {2577--2592},
	Publisher = {OUP},
	Title = {Min-type Morse theory for configuration spaces of hard spheres},
	Volume = {2014},
	Year = {2014}}

@article{Kahle2021configuration,
	Author = {Alpert, Hannah and Kahle, Matthew and MacPherson, Robert},
	Date-Modified = {2023-03-09 22:18:00 -0600},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {357--390},
	Publisher = {Springer},
	Title = {Configuration spaces of disks in an infinite strip},
	Volume = {5},
	Year = {2021}}

@article{alpert2020configuration,
	Author = {Alpert, Hannah and Bauer, Ulrich and Kahle, Matthew and MacPherson, Robert and Spendlove, Kelly},
	Journal = {arXiv preprint arXiv:2010.14480},
	Title = {Configuration spaces of hard squares in a rectangle},
	Year = {2020}}

@article{nazarova1975partially,
	Author = {Nazarova, Lyudmila Aleksandrovna},
	Journal = {Mathematics of the USSR-Izvestiya},
	Number = {5},
	Pages = {911},
	Publisher = {IOP Publishing},
	Title = {Partially ordered sets of infinite type},
	Volume = {9},
	Year = {1975}}

@article{miller2020homological,
      title={Homological algebra of modules over posets}, 
      author={Ezra Miller},
      year={2020},
      eprint={2008.00063},
      archivePrefix={arXiv}}

@article{kleiner1972partially,
	Author = {Kleiner, MM},
	Journal = {Zapiski Nauchnykh Seminarov POMI},
	Pages = {32--41},
	Publisher = {St. Petersburg Department of Steklov Institute of Mathematics, Russian~{\ldots}},
	Title = {Partially ordered sets of finite type},
	Volume = {28},
	Year = {1972}}

@inproceedings{edelsbrunner2000topological,
	Author = {Edelsbrunner, Herbert and Letscher, David and Zomorodian, Afra},
	Booktitle = {Proceedings 41st annual symposium on foundations of computer science},
	Organization = {IEEE},
	Pages = {454--463},
	Title = {Topological persistence and simplification},
	Year = {2000}}


@article{skryzalin2017numeric,
	Author = {Skryzalin, Jacek and Carlsson, Gunnar},
	Journal = {Journal of Applied and Computational Topology},
	Number = {1},
	Pages = {89--119},
	Publisher = {Springer},
	Title = {Numeric invariants from multidimensional persistence},
	Volume = {1},
	Year = {2017}}

@inproceedings{carlsson2009computing,
	Author = {Carlsson, Gunnar and Singh, Gurjeet and Zomorodian, Afra},
	Booktitle = {International Symposium on Algorithms and Computation},
	Organization = {Springer},
	Pages = {730--739},
	Title = {Computing multidimensional persistence},
	Year = {2009}}

@inproceedings{robins1999towards,
	Author = {Robins, Vanessa},
	Booktitle = {Topology proceedings},
	Number = {1},
	Pages = {503--532},
	Title = {Towards computing homology from finite approximations},
	Volume = {24},
	Year = {1999}}

	
@article{asashiba2018interval,
  title={On interval decomposability of 2D persistence modules},
  author={Asashiba, Hideto and Buchet, Micka{\"e}l and Escolar, Emerson G and Nakashima, Ken and Yoshiwaki, Michio},
  journal={Computational Geometry},
  volume={105},
  pages={101879},
  year={2022},
  publisher={Elsevier}
}	
	
	

@article{botnan2022introduction,
	Author = {Botnan, Magnus Bakke and Lesnick, Michael},
	Journal = {arXiv preprint arXiv:2203.14289},
	Title = {An introduction to multiparameter persistence},
	Year = {2022}}

@article{lesnick2015interactive,
	Author = {Lesnick, Michael and Wright, Matthew},
	Journal = {arXiv preprint arXiv:1512.00180},
	Title = {Interactive visualization of 2-d persistence modules},
	Year = {2015}}

@article{lesnick2022computing,
	Author = {Lesnick, Michael and Wright, Matthew},
	Journal = {SIAM Journal on Applied Algebra and Geometry},
	Number = {2},
	Pages = {267--298},
	Publisher = {SIAM},
	Title = {Computing minimal presentations and bigraded betti numbers of 2-parameter persistent homology},
	Volume = {6},
	Year = {2022}}

@book{weibel1995introduction,
	Author = {Weibel, Charles A},
	Number = {38},
	Publisher = {Cambridge university press},
    Address	 = "{C}ambridge",
	Title = {An introduction to homological algebra},
	Year = {1995}}

@book{rotman2009introduction,
	Author = {Rotman, Joseph J},
	Publisher = {Springer},
    Address	 = "New {Y}ork",
	Title = {An introduction to homological algebra},
	Volume = {2},
	Year = {2009}}

@book{brown2012cohomology,
  title={Cohomology of groups},
  author={Brown, Kenneth S},
  volume={87},
  year={2012},
  Address	 = "New {Y}ork",
  publisher={Springer Science \& Business Media}
}
	
@book{hatcher2002algebraic,
  title={Algebraic Topology},
  author={Hatcher, Allen},
  year={2002},
  publisher={Cambridge University Press}
}


==> chapters/chapter3.tex <==
\section{Equivalences of Categories}\label{equiv:cats}
It is known that the category of $1$-parameter persistence modules $\cat{Vect}_{\mathbb{F}}^{(\mathbb{R},\leq)}$ is equivalent to the category of modules over the monoid ring generated by $x^\alpha$, where $\alpha\in\mathbb{R}$. In particular, $\cat{Vect}_{\mathbb{F}}^{(\mathbb{Z},\leq)}$ is equivalent to the category of the modules over the polynomial ring $\mathbb{F}[x]$.

%$\mathbb{R}$-graded $\mathbb{F}\mathbb{R}_{\geq 0}$-modules $\cat{Gr}^{\mathbb{R}}\cat{Mod}_{\mathbb{FR}_{\geq 0}}$, where $\mathbb{F}\mathbb{R}_{\geq 0}$ is the monoid algebra of $\mathbb{R}_{\geq 0}$ over $\mathbb{F}$. The latter category is the $\mathbb{R}$-graded module over the algebra generated by the monomials of the form $x^a$ where $a\in \mathbb{R}_{\geq 0}$. \\

This fact can be generalized as follows: Let $\cat{C}$ be a small category and $R$ be a commutative ring. Define $$R\cat{C}=\{\sum a_i f_i\mid a_i\in R, a_i\neq 0 \mbox{ for finitely many $i$, }  f_i\in\mor{\cat{C}}\}$$
In other words, $R\cat{C}$, as a set, consists of all formal linear combinations of the form $\sum\limits_{i} a_i f_i$. Equip $R\cat{C}$ the binary operation: for $f,g\in\mor{\cat{C}}$,
$$f\cdot g=\begin{cases} f\circ g, & \mbox{if the range of $g$ is the domain of $f$; }  \\ 0, & \mbox{else } \end{cases}$$
Extend it linearly, we obtain
$$\sum\limits_{i} a_i f_i\cdot \sum\limits_{j} b_j g_j=\sum\limits_{i,j} (a_ib_j) f_i\cdot g_j$$
On the other hand, for any $c\in R$ and $\sum\limits_{i} a_i f_i\in R\cat{C}$, define $$c\cdot \sum\limits_{i} a_i f_i= \sum\limits_{i} (ca_i) f_i$$
$R\cat{C}$ with the above binary operation and scalar multiplication is called the \textbf{category algebra}\index{category algebra} of $\cat{C}$.
\begin{proposition}
Let $\cat{C}$ be a small category and $\mathbb{F}$ be a field. Then there exists a fully faithful functor $$\cat{Vect}_{\mathbb{F}}^{\cat{C}}\rightarrow \cat{Mod}_{\mathbb{F}\cat{C}}$$ 
\end{proposition}
\begin{proof}
Define $\Phi: \cat{Vect}_{\mathbb{F}}^{\cat{C}}\rightarrow \cat{Mod}_{\mathbb{F}\cat{C}}$ as follows:
\begin{description}
\item[ At the object level ]  Given $M\in \cat{Vect}_{\mathbb{F}}^{\cat{C}}$, define $\Phi(M)=\bigoplus\limits_{c\in \ob\cat{C}} Mc$. Note that $\Phi(M)$ is well-defined as a vector space\footnote{Because $\cat{Vect}_{\mathbb{F}}$ is complete and cocomplete.}. Define an $\mathbb{F}\cat{C}$-action on $\bigoplus\limits_{c\in \ob\cat{C}} Mc$: it suffices to define the $\mathbb{F}\cat{C}$-action coordinate-wise, then extend it linearly. 

Given $c,d\in\ob\cat{C}$ and $f\in\hom_\cat{C}(c,d)$, define $f_c=\inc_{d}\circ Mf\circ\proj_c$, i.e., $f_c$ is the composition of the morphisms in the diagram:
$$\bigoplus\limits_{c\in \ob\cat{C}} Mc\xrightarrow{\proj_c}  Mc\xrightarrow{M(c\xrightarrow{f} d)} M_{d}\xrightarrow{inc_{d}} \bigoplus\limits_{c\in \ob\cat{C}} Mc$$
For any $x\in\bigoplus\limits_{c\in \ob\cat{C}} Mc$ and $f\in\hom_\cat{C}(c,d)$, define $$f\cdot x=f_c(x) $$
This construction gives a ring action on $\Phi(M)$: given $f\in\hom_\cat{C}(c,d)$, $g\in\hom_\cat{C}(d,e)$, and $x\in \Phi(M)$, 
\begin{equation}
\begin{aligned}
g(f(x))&=g(f_c(x))=g_d(f_c(x))\\
&=\inc_{e}\circ Mg\circ\proj_{d}\circ\inc_{d}\circ Mf\circ\proj_c\\
&=\inc_{e}\circ Mg\circ(\proj_{d}\circ\inc_{d})\circ Mf\circ\proj_c\\
&=\inc_{e}\circ Mg\circ Mf\circ\proj_c\\
&=\inc_{e}\circ M(g\circ f)\circ\proj_c\\
&=(g\circ f)\cdot x
\end{aligned}
\end{equation}





\item[ At the morphism level ] Let $\alpha: M\Rightarrow N$ be a morphism in $\cat{Vect}_{\mathbb{F}}^{\cat{C}}$. Let $\Phi(\alpha)$ denote the yet-to-be-defined morphism in $\cat{Mod}_{\mathbb{F}\cat{C}}$ corresponding to $\alpha$. As a morphism in $\cat{Vect}_{\mathbb{F}}$, we are forced to define $\Phi(\alpha)=(\alpha_c)_{c\in \ob\cat{C}}$. Note that $\Phi(\alpha)$ is an $\mathbb{F}\cat{C}$-morphism: it suffices to show that for every $f\in \mor\cat{C}$, $\Phi(\alpha)(f\cdot x)=f\cdot\Phi(\alpha)(x)$ for all $x\in\bigoplus\limits_{c\in \ob\cat{C}} Mc$. By the naturality of $\alpha$, we have
$$\mathcal{N}f\circ \alpha_c=\alpha_{d}\circ Mf, \mbox{ if the source of $f$ is $c$ and the target of $f$ is $d$}$$
Hence 
\begin{equation}
\begin{aligned}
f\cdot\Phi(\alpha)(x)&=\inc_{d}\circ Nf\circ\proj_c\circ \Phi(\alpha)(x)\\
&=\inc_{d}\circ Nf\circ\alpha_c\circ \proj_c(x)\\
&=\inc_{d}\circ \alpha_d\circ Mf\circ \proj_c(x)\\
&=\Phi(\alpha)\circ \inc_d\circ Mf\circ \proj_c(x)\\
&=\Phi(\alpha) (f\cdot x)
\end{aligned}
\end{equation}
\end{description}

Now we are going to show 
\begin{equation*}
\begin{aligned}
\phi:\hom(M, N)&\rightarrow \hom(\bigoplus\limits_{c\in \ob\cat{C}} Mc, \bigoplus\limits_{c\in \ob\cat{C}} Nc)\\ 
\alpha&\mapsto \Phi(\alpha)=(\alpha_c)_{c\in\ob\cat{C}}
 \end{aligned}
\end{equation*}
 is a bijection for every $M,N\in\cat{Vect}_{\mathbb{F}}^{\cat{C}}$. The well-definedness and injectivity of $\phi$ is clear by the universal property of the coproduct. Now we are going to show that $\phi$ is surjective. Given $(f_c)_{c\in \ob\cat{C}}:\bigoplus\limits_{c\in \ob\cat{C}} Mc\rightarrow\bigoplus\limits_{c\in \ob\cat{C}} Nc$, define $\alpha:M\Rightarrow N$ by $\alpha_c=f_c$ for all $c\in \ob\cat{C}$. Consider the following diagram:
 \begin{center}
 \begin{tikzcd}
  Mc \arrow{r}{\inc_c} \arrow{d}{f_c}
        & \bigoplus\limits_{c\in \ob\cat{C}} Mc \arrow{r}{f\cdot}\arrow{d}{(f_c)_{c\in \ob\cat{C}}} & \bigoplus\limits_{c\in \ob\cat{C}} Mc \arrow{r}{\proj_{d}}\arrow{d}{(f_c)_{c\in \ob\cat{C}}} & Md  \arrow{d}{f_{d}} \\
  Nc \arrow{r}{\inc_c}
 &\bigoplus\limits_{c\in \ob\cat{C}} Nc\arrow{r}{f\cdot} & \bigoplus\limits_{c\in \ob\cat{C}} Nc\arrow{r}[color=black]{\proj_{d}} & Nd \\
\end{tikzcd}
 \end{center}
 Note that each small square of the above diagram is commutative: 
 \begin{itemize}
\item the square on the left is commutative by the universal property of coproducts,
\item the square on the right is commutative since the horizontal arrows are projection maps,
\item the square in the middle is commutative since $(f_c)_{c\in \ob\cat{C}}$ is an $\mathbb{F}\cat{C}$-homomorphism.
\end{itemize}

Therefore, the outer square is commutative. Note that the composition of the morphisms in the top row is $Mf$ because
\begin{equation}
\begin{aligned}
\proj_{d}\circ f\circ \inc_c(y)&=\proj_{d}\circ f_c (\inc_c(y))\\
&=\proj_{d}\circ \inc_d \circ Mf\circ \proj_c\circ \inc_c(y)\\
&=Mf(y)
\end{aligned}
\end{equation}
Similarly, the composition of the morphisms in the bottom row is $Nf$. Hence we obtain the following commutative diagram for all $g\in G$ and $s\in S$:
 \begin{center}
 \begin{tikzcd}
Mc\arrow{r}{Mf} \arrow{d}{f_c}
        & Md \arrow{d}{f_{d}} \\
  Nc \arrow{r}{Nf}
 & Nd \\
\end{tikzcd}
 \end{center}
Therefore, $\alpha$ is a natural transformation.
\end{proof}

As a consequence, $\cat{Vect}_{\mathbb{F}}^{\cat{C}}$ is equivalent to a full subcategory of $\cat{Mod}_{\mathbb{F}\cat{C}}$.\\





==> ldr-article.tex <==
\LoadClass[letter,10pt,notitlepage]{article}
%\usepackage{microtype}
\usepackage{setspace}
%\singlespacing
%\onehalfspacing
\usepackage{lipsum}%put paragraph into a box
\usepackage{amsfonts}
\usepackage{amsmath,amscd,amssymb}
\usepackage{mathrsfs}%use: \mathscr{FP}
\usepackage{amsthm,xcolor}
\usepackage{mathtools}% To colour equation numbers in proof
\usepackage{extarrows}
\usepackage[all,cmtip]{xy}
\usepackage{mbboard}%category Bolded font. e.g. $\bbDelta$
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage[toc,page]{appendix}
\usepackage{enumitem, calc}%change align of description environment e.g. \begin{description}[labelwidth= \widthof{\bfseries Long long E3:}, align =right] item[E1:] Example item 1 \item[Long long E3:] Example item 3 \end{description}
\usepackage{graphicx}
%\usepackage[top=2.5cm,bottom=2.5cm,left=2cm,right=2  cm,dvips]{geometry}
\usepackage[paperheight=27cm,top=2cm, bottom=2cm, left=1.5cm, right=1.5cm,dvips]{geometry}
\usepackage{marginnote}%sidenotes on the right. To make it on the left, use \reversemarginpar
\usepackage{fontspec}
%\usepackage[dvips]
\usepackage{empheq}%emphasis yellow box \begin{shaded}\end{shaded}
\usepackage{framed}
\usepackage[most]{tcolorbox}
\usepackage{xcolor}
\colorlet{shadecolor}{orange!15}
\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{dsfont}%bolded math font %%%%%%%%%%%% E.g.  \mathds{1}
\usepackage{titlesec} 
\usepackage{titletoc} 
\usepackage{mdframed}
\usepackage{indentfirst} 
%\usepackage{tocbibind}%include contents on the table of contents
\usepackage{erewhon}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{mathpazo}
\setmainfont
     [BoldFont       = texgyrepagella-bold.otf ,
       ItalicFont     = texgyrepagella-italic.otf ,
       BoldItalicFont = texgyrepagella-bolditalic.otf ]
     {texgyrepagella-regular.otf}
%%%% A simple MakeIndex style

%%% end
%\usepackage{xypic}
\usepackage[
backend=biber,
style=alphabetic,
sorting=nyt,maxbibnames=99]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
\addbibresource{app.bib}%
\usepackage[small,nohug,heads=LaTeX]{diagrams}
\diagramstyle[labelstyle=\scriptstyle]
\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{shapes.geometric, positioning, calc}
\usetikzlibrary{arrows}
\usetikzlibrary{graphs}
\usepackage{pgfplots}
\usetikzlibrary{3d,calc}
\usepackage{gensymb}
\usepackage{graphics,graphicx} 
%\usepackage{pstricks,pst-node,pst-tree}
%\usepackage{pst-plot} 
\usepackage{stmaryrd}% provides \mapsfrom
\usepackage{textcomp,booktabs}
\usepackage{soul} %strikethrough text. \st{} %also highilght text \hl{}
\usepackage{colortbl}
\usepackage{spectralsequences}
\usepackage{caption}
\usepackage{smartdiagram}%flowchart
\usepackage{mwe}
\usepackage[colorlinks,
            linkcolor=blue,
            anchorcolor=blue,
            citecolor=blue,
            urlcolor=blue,
            ]{hyperref}
\usepackage{pstricks-add}
\usepackage{pst-solides3d}
\usepackage{pst-plot}
\usepackage{pst-poly}
\usepackage{color}
\definecolor{myblue}{rgb}{.8, .8, 1}
\usepackage{babel}
\usepackage{amsmath}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\colim}{colim}
\newcommand{\cat}[1]{\mathbf{\boldsymbol{\mathsf{#1}}}}
\usepackage{empheq}

\newlength\mytemplen
\newsavebox\mytempbox

\makeatletter
\newcommand\mybluebox{%
    \@ifnextchar[%]
       {\@mybluebox}%
       {\@mybluebox[0pt]}}

\def\@mybluebox[#1]{%
    \@ifnextchar[%]
       {\@@mybluebox[#1]}%
       {\@@mybluebox[#1][0pt]}}

\def\@@mybluebox[#1][#2]#3{
    \sbox\mytempbox{#3}%
    \mytemplen\ht\mytempbox
    \advance\mytemplen #1\relax
    \ht\mytempbox\mytemplen
    \mytemplen\dp\mytempbox
    \advance\mytemplen #2\relax
    \dp\mytempbox\mytemplen
    \colorbox{myblue}{\hspace{1em}\usebox{\mytempbox}\hspace{1em}}}
\makeatother %highlight formula \begin{emphep}[box={\mybluebox[5pt]}]{equayion*}\end{emphep}
\usetikzlibrary{positioning}
%\definecolor{mycolor}{rgb}{0.5, 0.1, 0.2}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}%For restriction of a function. Type #\restr{f}{A}
\let\oldproof\proof
\renewcommand{\proof}{\color{black}\oldproof} %change proof color here
\renewcommand{\baselinestretch}{1}\normalsize
\makeatletter
\newcommand\tline[2]{$\underset{\text{#1}}{\text{\underline{\hspace{#2}}}}$}
\renewcommand{\ker}{\mathsf{ker}}
\renewcommand{\lim}{\mathsf{lim}}
\renewcommand{\colim}{\mathsf{colim}}
\renewcommand{\hom}{\hspace{0.1em}\mathsf{Hom}}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newcommand{\highlight}[3][black]{{\fboxsep0.5pt\colorbox{#2}{\color{#1} #3}}} %\highlight[white]{blue!50}{} %%%highlighting word or sentence
\theoremstyle{definition}
\DeclareMathOperator{\op}{\hspace{-0.2em}^{\mathsf{op}}}
\DeclareMathOperator{\proj}{\mathsf{proj}}
\DeclareMathOperator{\inc}{\mathsf{inc}}
\DeclareMathOperator{\coker}{\mathsf{coker}}
\DeclareMathOperator{\id}{\mathsf{id}}
\DeclareMathOperator{\End}{\mathsf{End}}
\DeclareMathOperator{\rank}{\mathsf{rank}}
\DeclareMathOperator{\diam}{\mathsf{diam}}%diameter of the graph
\newtheorem{examplex}{Example}
\newenvironment{example}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}\examplex}
  {\popQED\endexamplex}
\newtheorem{lemma}{Lemma}
\newtheorem*{pflemma}{\indent Proof of lemma}
\let\oldpflemma\pflemma
\renewcommand{\pflemma}{\color{black}\oldpflemma}%change the color of proof of lemma 
\newcommand*{\QEDlemma}{\hfill\ensuremath{\blacksquare}}
\newtheorem{proposition}[theorem]{Proposition}
\newcommand{\compactlist}{\setlength{\itemsep}{0pt} \setlength{\parskip}{0pt} \setlength{\leftskip}{-1em}}
\newcommand*{\Resize}[2]{\resizebox{#1}{!}{$#2$}}%recale the formula. Eg $$ \Resize{1cm}{y = \sin^2 x}$$
\newcommand{\ds}{\displaystyle}
\newcommand{\blank}{\underline{\hspace{2cm}}}
\makeatletter
\DeclareMathOperator{\Ima}{\mathsf{Im}}
\DeclareMathOperator{\mor}{\mathsf{mor}}
\DeclareMathOperator{\ob}{\mathsf{ob}}
\makeatletter
\newcommand\dirlim{\mathop{\mathpalette\varlim@{\rightarrowfill@\scriptstyle}}\nmlimits@}
\newcommand\invlim{\mathop{\mathpalette\varlim@{\leftarrowfill@\scriptstyle}}\nmlimits@}
\makeatother
\newtheorem*{remark}{Remark}
\newtheorem*{solution}{Solution}
\let\oldsolution\solution
\renewcommand{\solution}{\color{black}\oldsolution}%change proof color here
\diagramstyle[labelstyle=\scriptstyle]
\colorlet{mycolor}{blue!100}
\newmdenv[linecolor=mycolor,skipabove=\topsep,skipbelow=\topsep,
leftmargin=5pt,rightmargin=5pt,
innerleftmargin=5pt,innerrightmargin=5pt]{mybox}
\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}
\newcommand\polygon[2][]{
  \pgfmathsetmacro{\angle}{360/#2}
  \pgfmathsetmacro{\startangle}{-90 + \angle/2}
  \pgfmathsetmacro{\y}{cos(\angle/2)}
  \begin{scope}[#1]
    \foreach \i in {1,2,...,#2} {
      \pgfmathsetmacro{\x}{\startangle + \angle*\i}
      \draw[fill=blue!15] (0, 0) -- (\x:1 cm) -- (\x + \angle/2:\y cm) -- cycle;
      \draw[fill=blue!30] (0, 0) -- (\x + \angle/2:\y cm) -- (\x + \angle:1 cm) -- cycle;
    }
  \end{scope}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup\lccode`~=`& \lowercase{\endgroup
\newcommand{\spmat}[1]{%
  \left[
  \let~=&
  \begin{smallmatrix}#1\end{smallmatrix}
  \right]
}}


% Title page font
\newcommand{\titlepagefontsize}{\fontsize{10}{12}\selectfont}
\newcommand{\titlefont}{\fontfamily{SourceSansPro-LF}\bfseries\fontsize{16}{18}\selectfont}

%Put abstract header on same line as abstract, define font size
\renewenvironment{abstract}%
		 {%
		  \begin{list}{}%
		     {\setlength{\rightmargin}{2cm}%
		      \setlength{\leftmargin}{2cm}}%
		   \item[]\ignorespaces%
		   \titlepagefontsize
		   \textbf{Abstract:}}%
		 {\unskip\end{list}}
		 
% Define additional title page commands
\makeatletter
\def\keywords{\xdef\@thefnmark{}\@footnotetext}
\makeatother

\newcommand{\correspondingauthor}[1]{\titlepagefontsize\textbf{Corresponding author: }#1 \\[\baselineskip]}

\newcommand{\orcid}[1]{\titlepagefontsize\textbf{ORCID ID: }\url{#1} \\[\baselineskip]}

\newcommand{\citationinfo}[1]{\titlepagefontsize\textbf{Citation: }#1 \\[\baselineskip]%
% The end of title page is after the end of the citation info. We add a page break and return to the normal font size
\clearpage\normalsize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lhead{}
\rhead{}
\chead[]{}
\lfoot{}

\rfoot{Page \thepage \hspace{1pt} of \pageref{LastPage}}

%\pagestyle{fancy}

